Unlocking Generalization Power in LiDAR Point Cloud Registration

In real-world environments, a LiDAR point cloud registration method with robust generalization capabilities (across varying distances and datasets) is crucial for ensuring safety in autonomous driving and other LiDAR-based applications. However, current methods fall short in achieving this level of generalization. To address these limitations, we propose UGP, a pruned framework designed to enhance generalization power for LiDAR point cloud registration. The core insight in UGP is the elimination of cross-attention mechanisms to improve generalization, allowing the network to concentrate on intra-frame feature extraction. Additionally, we introduce a progressive self-attention module to reduce ambiguity in large-scale scenes and integrate Bird's Eye View (BEV) features to incorporate semantic information about scene elements. Together, these enhancements significantly boost the network's generalization performance. We validated our approach through various generalization experiments in multiple outdoor scenes. In cross-distance generalization experiments on KITTI and nuScenes, UGP achieved state-of-the-art mean Registration Recall rates of 94.5% and 91.4%, respectively. In cross-dataset generalization from nuScenes to KITTI, UGP achieved a state-of-the-art mean Registration Recall of 90.9%. Code will be available at https://github.com/peakpang/UGP.

==> sec/2_related_work.tex <==
\section{Related Work}
\label{sec:Related Work}
%-------------------------------------------------------------------------
\begin{figure*}[t]
    \centering
    \includegraphics [width=1\linewidth]{sec/fig/motivation.pdf}
    \caption{\textbf{Motivation.} We conducted a statistical analysis of the matching characteristics in LiDAR scenes and identified the limitations of existing methods. This was followed by preliminary visualizations and elimination experiments to validate our findings. (a) Each point in the figure represents a ground truth corresponding superpoint pair. The position of each point indicates the neighborhood count (NC) of the superpoint within a radius of $r=2.4m$ in both the source (src) and target (tgt) point clouds, and the color represents the overlap degree of the corresponding superpoint pairs after rotation by the ground truth transformation. (b) Performance of existing methods in cross-distance (upper left) and cross-dataset (upper right). (c) GeoTrans \cite{qin2022geometric} cannot match superpoints (cross-distance, from KITTI@10m to KITTI@20m). (d) The performance of existing methods after eliminating cross-attention, and UGP (ours).
    }
    \label{fig:motivation}
\end{figure*}
%-------------------------------------------------------------------------
\noindent\textbf{Learning-based Point Cloud Registration.} Learning-based point cloud registration methods have become a powerful approach for aligning point clouds. Current methods often employ a coarse-to-fine strategy \cite{yu2021cofinet,qin2022geometric,yu2023rotation,yu2023peal,chen2024dynamic,yao2024pare,mu2024colorpcr,xiong2024speal}, which loosens the constraints of strict point-to-point matching in favor of patch-level matching. This approach reduces repeatability requirements, significantly enhancing registration accuracy. However, these methods rely heavily on the data distribution of training point cloud pairs, which limits their generalization capability. Following this line, point-wise methods \cite{choy2019fully,bai2020d3feat} utilize architectures such as Minkowski \cite{Minkowski2019} and KPConv \cite{thomas2019kpconv} to extract dense point features, while patch-wise methods \cite{deng2018ppfnet,gojcic2019perfect,ao2021spinnet,GeDi2022,ao2023buffer} capture features from the local regions around key points through carefully designed networks. The robustness of local patches to noise and occlusion gives these patch-based approaches a promising generalization potential. Recent studies \cite{liu2023apr,liu2023density, liu2024extend} have focused on point cloud registration across varying distances. However, these approaches rely solely on visible full-range data and require carefully designed multi-frame training to ensure registration performance within the visible range.

\noindent\textbf{Point Cloud Registration with Transformers.} The Transformer architecture \cite{vaswani2017attention} introduced an attention mechanism that captures global dependencies and has been widely used for point cloud registration. For example, CoFiNet \cite{yu2021cofinet} uses vanilla attention mechanism to establish global geometric consistency, while GeoTrans \cite{qin2022geometric} integrates geometric structure to enhance feature robustness. PEAL \cite{yu2023peal} employs one-way attention with overlap priors to reduce ambiguity from non-overlapping points. DCATr \cite{chen2024dynamic} limits attention to specific cues to minimize irrelevant interference. Unlike these methods, we propose a progressive self-attention mechanism that gradually expands the spatial attention range, prioritizing finer local spatial structure associations, reducing ambiguity in large scenes, and improving registration accuracy.

%-------------------------------------------------------------------------
\noindent\textbf{Multi-modal Point Cloud Registration.} Incorporating multi-modal information for point cloud understanding has gained significant traction in recent research. For example, RPVNet \cite{xu2021rpvnet} enhances segmentation accuracy by integrating the range image modality. Methods such as BYOC \cite{el2021bootstrap}, PCRCG \cite{zhang2022pcr}, and IGReg \cite{xu2024igreg} fuse image features with point clouds to support registration tasks. Similarly, PEAL2D \cite{yu2023peal} utilizes a 2D image to derive an overlap prior, aiding in point cloud registration. BEV images, widely adopted in 3D object detection \cite{Yang_2018_CVPR} and place recognition~\cite{luo2023bevplace}, are particularly effective due to their clear global edge features. To enhance matching accuracy in the coarse stage, we explicitly incorporate BEV images into point cloud registration. 









